Higher order quantization conditions for two-body scattering with spin

We examine the L\"uscher quantization condition to high order for the scattering of a spinless particle and a spin-1/2 particle in a periodic box. First, we derive the quantization conditions in a non-relativistic framework up to total angular momentum $J=11/2$ in both cubic and elongated geometries, and for both rest and moving frames. Then, we introduce a method to transparently cross-check their convergence, using both quantized energy levels in the box and infinite-volume phase shifts for the same potential. We clarify how to incorporate spin-orbit coupling into the formalism and show in detail how the quantization conditions converge order by order in the various irreducible representations. In all, we validated 19 quantization conditions (12 in cubic box, 7 in elongated box). This is a necessary step in applying the method in precision studies of systems in finite volume with half-integer spin, such as meson-baryon scattering.

==> Tables/BasisVectors/Temp.tex <==
\begin{longtable}{CCCCCC|CCCCCC}
\caption{\comm{make this table two columns to fit the page} Basis vectors of $^2D_{4h}$ in terms of spi spherical harmonics $Y(J,M)$ up to $J = \frac{13}{2}$ for the rest frame of the elongated box. Multiplicities are labeled by $n$ and multidimensional components are indicated by $\alpha$.}
\label{tab:elongatedbasisvectors}
\renewcommand{\arraystretch}{2.0}
\endfirsthead
\hline \endhead
\hline \\ \endfoot
\hline \\ \endlastfoot
\toprule
 \Gamma  & \text{J} & \text{l} & \text{n} & \alpha  & \text{Basis Vector} & \Gamma  & \text{J} & \text{l} & \text{n} & \alpha  & \text{Basis Vector} \\
 \text{G1g} & \frac{1}{2} & 0 & 1 & 1 & Y\left(\frac{1}{2},\frac{1}{2}\right) & \text{G1u} & \frac{1}{2} & 1 & 1 & 1 & Y\left(\frac{1}{2},\frac{1}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{1}{2},-\frac{1}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{1}{2},-\frac{1}{2}\right) \\
 \text{G1g} & \frac{3}{2} & 2 & 1 & 1 & Y\left(\frac{3}{2},\frac{1}{2}\right) &\text{G1u} & \frac{3}{2} & 1 & 1 & 1 & Y\left(\frac{3}{2},\frac{1}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{3}{2},-\frac{1}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{3}{2},-\frac{1}{2}\right) \\
 \text{G1g} & \frac{5}{2} & 2 & 1 & 1 & Y\left(\frac{5}{2},\frac{1}{2}\right) & \text{G1u} & \frac{5}{2} & 3 & 1 & 1 & Y\left(\frac{5}{2},\frac{1}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{5}{2},-\frac{1}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{5}{2},-\frac{1}{2}\right) \\
 \text{G1g} & \frac{7}{2} & 4 & 1 & 1 & Y\left(\frac{7}{2},-\frac{7}{2}\right) & \text{G1u} & \frac{7}{2} & 3 & 1 & 1 & Y\left(\frac{7}{2},-\frac{7}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{7}{2},\frac{7}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{7}{2},\frac{7}{2}\right) \\
 \text{G1g} & \frac{7}{2} & 4 & 2 & 1 & Y\left(\frac{7}{2},\frac{1}{2}\right) & \text{G1u} & \frac{7}{2} & 3 & 2 & 1 & Y\left(\frac{7}{2},\frac{1}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{7}{2},-\frac{1}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{7}{2},-\frac{1}{2}\right) \\
 \text{G1g} & \frac{9}{2} & 4 & 1 & 1 & Y\left(\frac{9}{2},-\frac{7}{2}\right) &  \text{G1u} & \frac{9}{2} & 5 & 1 & 1 & Y\left(\frac{9}{2},-\frac{7}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{9}{2},\frac{7}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{9}{2},\frac{7}{2}\right) \\
 \text{G1g} & \frac{9}{2} & 4 & 2 & 1 & Y\left(\frac{9}{2},\frac{1}{2}\right) & \text{G1u} & \frac{9}{2} & 5 & 2 & 1 & Y\left(\frac{9}{2},\frac{1}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{9}{2},-\frac{1}{2}\right) &  \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{9}{2},-\frac{1}{2}\right) \\
 \text{G1g} & \frac{9}{2} & 4 & 3 & 1 & Y\left(\frac{9}{2},\frac{9}{2}\right) &  \text{G1u} & \frac{9}{2} & 5 & 3 & 1 & Y\left(\frac{9}{2},\frac{9}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{9}{2},-\frac{9}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{9}{2},-\frac{9}{2}\right) \\
 \text{G1g} & \frac{11}{2} & 6 & 1 & 1 & Y\left(\frac{11}{2},-\frac{7}{2}\right) & \text{G1u} & \frac{11}{2} & 5 & 1 & 1 & Y\left(\frac{11}{2},-\frac{7}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{11}{2},\frac{7}{2}\right) &  \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{11}{2},\frac{7}{2}\right) \\
 \text{G1g} & \frac{11}{2} & 6 & 2 & 1 & Y\left(\frac{11}{2},\frac{1}{2}\right) & \text{G1u} & \frac{11}{2} & 5 & 2 & 1 & Y\left(\frac{11}{2},\frac{1}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{11}{2},-\frac{1}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{11}{2},-\frac{1}{2}\right) \\
 \text{G1g} & \frac{11}{2} & 6 & 3 & 1 & Y\left(\frac{11}{2},\frac{9}{2}\right) & \text{G1u} & \frac{11}{2} & 5 & 3 & 1 & Y\left(\frac{11}{2},\frac{9}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{11}{2},-\frac{9}{2}\right) &  \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{11}{2},-\frac{9}{2}\right) \\
 \text{G1g} & \frac{13}{2} & 6 & 1 & 1 & Y\left(\frac{13}{2},-\frac{7}{2}\right) & \text{G1u} & \frac{13}{2} & 7 & 1 & 1 & Y\left(\frac{13}{2},-\frac{7}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{13}{2},\frac{7}{2}\right) &  \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{13}{2},\frac{7}{2}\right) \\
 \text{G1g} & \frac{13}{2} & 6 & 2 & 1 & Y\left(\frac{13}{2},\frac{1}{2}\right) & \text{G1u} & \frac{13}{2} & 7 & 2 & 1 & Y\left(\frac{13}{2},\frac{1}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{13}{2},-\frac{1}{2}\right) &  \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{13}{2},-\frac{1}{2}\right) \\
 \text{G1g} & \frac{13}{2} & 6 & 3 & 1 & Y\left(\frac{13}{2},\frac{9}{2}\right) & \text{G1u} & \frac{13}{2} & 7 & 3 & 1 & Y\left(\frac{13}{2},\frac{9}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{13}{2},-\frac{9}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{13}{2},-\frac{9}{2}\right) \\
 \hline

 \text{G2g} & \frac{3}{2} & 2 & 1 & 1 & Y\left(\frac{3}{2},-\frac{3}{2}\right) & \text{G2u} & \frac{3}{2} & 1 & 1 & 1 & Y\left(\frac{3}{2},-\frac{3}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{3}{2},\frac{3}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{3}{2},\frac{3}{2}\right) \\
 \text{G2g} & \frac{5}{2} & 2 & 1 & 1 & Y\left(\frac{5}{2},-\frac{3}{2}\right) & \text{G2u} & \frac{5}{2} & 3 & 1 & 1 & Y\left(\frac{5}{2},-\frac{3}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{5}{2},\frac{3}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{5}{2},\frac{3}{2}\right) \\
 \text{G2g} & \frac{5}{2} & 2 & 2 & 1 & Y\left(\frac{5}{2},\frac{5}{2}\right) & \text{G2u} & \frac{5}{2} & 3 & 2 & 1 & Y\left(\frac{5}{2},\frac{5}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{5}{2},-\frac{5}{2}\right) &  \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{5}{2},-\frac{5}{2}\right) \\
 \text{G2g} & \frac{7}{2} & 4 & 1 & 1 & Y\left(\frac{7}{2},-\frac{3}{2}\right) & \text{G2u} & \frac{7}{2} & 3 & 1 & 1 & Y\left(\frac{7}{2},-\frac{3}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{7}{2},\frac{3}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{7}{2},\frac{3}{2}\right) \\
 \text{G2g} & \frac{7}{2} & 4 & 2 & 1 & Y\left(\frac{7}{2},\frac{5}{2}\right) &  \text{G2u} & \frac{7}{2} & 3 & 2 & 1 & Y\left(\frac{7}{2},\frac{5}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{7}{2},-\frac{5}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{7}{2},-\frac{5}{2}\right) \\
 \text{G2g} & \frac{9}{2} & 4 & 1 & 1 & Y\left(\frac{9}{2},-\frac{3}{2}\right) & \text{G2u} & \frac{9}{2} & 5 & 1 & 1 & Y\left(\frac{9}{2},-\frac{3}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{9}{2},\frac{3}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{9}{2},\frac{3}{2}\right) \\
 \text{G2g} & \frac{9}{2} & 4 & 2 & 1 & Y\left(\frac{9}{2},\frac{5}{2}\right) &  \text{G2u} & \frac{9}{2} & 5 & 2 & 1 & Y\left(\frac{9}{2},\frac{5}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{9}{2},-\frac{5}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{9}{2},-\frac{5}{2}\right) \\
 \text{G2g} & \frac{11}{2} & 6 & 1 & 1 & Y\left(\frac{11}{2},-\frac{11}{2}\right) & \text{G2u} & \frac{11}{2} & 5 & 1 & 1 & Y\left(\frac{11}{2},-\frac{11}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{11}{2},\frac{11}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{11}{2},\frac{11}{2}\right) \\
 \text{G2g} & \frac{11}{2} & 6 & 2 & 1 & Y\left(\frac{11}{2},-\frac{3}{2}\right) & \text{G2u} & \frac{11}{2} & 5 & 2 & 1 & Y\left(\frac{11}{2},-\frac{3}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{11}{2},\frac{3}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{11}{2},\frac{3}{2}\right) \\
 \text{G2g} & \frac{11}{2} & 6 & 3 & 1 & Y\left(\frac{11}{2},\frac{5}{2}\right) & \text{G2u} & \frac{11}{2} & 5 & 3 & 1 & Y\left(\frac{11}{2},\frac{5}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{11}{2},-\frac{5}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & Y\left(\frac{11}{2},-\frac{5}{2}\right) \\
 \text{G2g} & \frac{13}{2} & 6 & 1 & 1 & Y\left(\frac{13}{2},-\frac{11}{2}\right) & \text{G2u} & \frac{13}{2} & 7 & 1 & 1 & Y\left(\frac{13}{2},-\frac{11}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{13}{2},\frac{11}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{13}{2},\frac{11}{2}\right) \\
 \text{G2g} & \frac{13}{2} & 6 & 2 & 1 & Y\left(\frac{13}{2},-\frac{3}{2}\right) & \text{G2u} & \frac{13}{2} & 7 & 2 & 1 & Y\left(\frac{13}{2},-\frac{3}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{13}{2},\frac{3}{2}\right) & \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{13}{2},\frac{3}{2}\right) \\
 \text{G2g} & \frac{13}{2} & 6 & 3 & 1 & Y\left(\frac{13}{2},\frac{5}{2}\right) & \text{G2u} & \frac{13}{2} & 7 & 3 & 1 & Y\left(\frac{13}{2},\frac{5}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{13}{2},-\frac{5}{2}\right) &  \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{13}{2},-\frac{5}{2}\right) \\
 \text{G2g} & \frac{13}{2} & 6 & 4 & 1 & Y\left(\frac{13}{2},\frac{13}{2}\right) & \text{G2u} & \frac{13}{2} & 7 & 4 & 1 & Y\left(\frac{13}{2},\frac{13}{2}\right) \\
 \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{13}{2},-\frac{13}{2}\right) &  \text{} & \text{} & \text{} & \text{} & 2 & -Y\left(\frac{13}{2},-\frac{13}{2}\right) \\
\end{longtable}

==> Tables/CubicG1gChi2Convergence.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{longtable*}{CCCCCCCCCCCCC}
\caption{Convergence of the higher order quantization conditions in the $G_{1g}$ irrep of the cubic rest frame by adding higher partial waves using the $\chi_2^2$ metric of comparing against the energy shift of the potential. All energies are given in $\GeV$.
\comm{attach last line to table 4 instead of whole new table. "Other levels converge to machine precision"}}
\label{tab:CubicG1gChi2Convergence}
\endfirsthead
\hline \endhead
\hline \\ \endfoot
\hline \\ \endlastfoot
\toprule
 \text{Level} & \text{Box L} & \text{Lattice} & \text{Order 1} & \text{Order 2} & \text{Order 3} & \text{Order 4} & \chi_2 ^2\text{ order 1} & \chi_2 ^2\text{ order 2} & \chi_2 ^2\text{ order 3} & \chi_2 ^2\text{ order 4} \\
 \hline
 1 & 0.00935738 & 0.00935737 & 0.00935738 & 0.00935738 & 0.00935738 & 0.00935738 & 2.14\times 10^{-16} & 1.28\times 10^{-16} & 1.24\times 10^{-14} & 1.24\times 10^{-14} \\
 2 & 0.0390926 & 0.0390926 & 0.0390923 & 0.0390924 & 0.0390926 & 0.0390926 & 5.97\times 10^{-9} & 3.73\times 10^{-9} & 1.15\times 10^{-15} & 1.26\times 10^{-15} \\
 3 & 0.0553602 & 0.0553602 & 0.05536 & 0.05536 & 0.0553602 & 0.0553602 & 1.65\times 10^{-9} & 1.03\times 10^{-9} & 1.06\times 10^{-12} & 8.82\times 10^{-13} \\
 4 & 0.0652422 & 0.0652422 & 0.065228 & 0.0652311 & 0.0652422 & 0.0652422 & 6.25\times 10^{-6} & 3.84\times 10^{-6} & 8.63\times 10^{-15} & 1.06\times 10^{-14} \\
 5 & 0.0716554 & 0.0716554 & 0.0716529 & 0.0716534 & 0.0716554 & 0.0716554 & 7.65\times 10^{-7} & 4.71\times 10^{-7} & 1.46\times 10^{-10} & 1.23\times 10^{-10} \\
 6 & 0.0769113 & 0.0769113 &  & 0.0768915 & 0.0769112 & 0.0769112 &  & 0.481 & 5.50\times 10^{-6} & 4.45\times 10^{-6} \\
 \bottomrule
\end{longtable*}

==> Tables/MatrixElements/Old.tex <==
\begin{longtable*}{CCCCCCCL}
\caption{Matrix elements for rest frame in cubic box (group $^2O_{h}$) up to the third partial wave in each irrep.
}
\label{tab:CubicRestMatrixElements}
\renewcommand{\arraystretch}{2.0}
\endfirsthead
\multicolumn{7}{c} {{\tablename\ \thetable{:} \it Continued}} \\
\hline \endhead
\hline \\ \endfoot
\hline \\ \endlastfoot
\toprule
\Gamma & J & l & n & J' & l' & n' & M^\Gamma_{Jln,J'l'n'} \\
\hline
  G_{1g} & \frac{1}{2} & 0 & 1 & \frac{1}{2} & 0 & 1 & \text{wr}_{0,0} \\
 \text{} & \frac{7}{2} & 4 & 1 & \frac{1}{2} & 0 & 1 & -\frac{4 \text{wr}_{4,0}}{\sqrt{21}} \\
 \text{} & \frac{7}{2} & 4 & 1 & \frac{7}{2} & 4 & 1 & \text{wr}_{0,0}+\frac{6 \text{wr}_{4,0}}{11}+\frac{100 \text{wr}_{6,0}}{33 \sqrt{13}} \\
 \text{} & \frac{9}{2} & 4 & 1 & \frac{1}{2} & 0 & 1 & 2 \sqrt{\frac{5}{21}} \text{wr}_{4,0} \\
 \text{} & \frac{9}{2} & 4 & 1 & \frac{7}{2} & 4 & 1 & -\frac{4}{7293} \left(153 \sqrt{5} \text{wr}_{4,0}+238 \sqrt{65} \text{wr}_{6,0}+168 \sqrt{85} \text{wr}_{8,0}\right) \\
 \text{} & \frac{9}{2} & 4 & 1 & \frac{9}{2} & 4 & 1 & \text{wr}_{0,0}+\frac{4}{7293} \left(1071 \text{wr}_{4,0}+544 \sqrt{13} \text{wr}_{6,0}+84 \sqrt{17} \text{wr}_{8,0}\right) \\
\hline
G_{1u} & \frac{1}{2} & 1 & 1 & \frac{1}{2} & 1 & 1 & \text{wr}_{0,0} \\
 \text{} & \frac{7}{2} & 3 & 1 & \frac{1}{2} & 1 & 1 & \frac{4 \text{wr}_{4,0}}{\sqrt{21}} \\
 \text{} & \frac{7}{2} & 3 & 1 & \frac{7}{2} & 3 & 1 & \text{wr}_{0,0}+\frac{6 \text{wr}_{4,0}}{11}+\frac{100 \text{wr}_{6,0}}{33 \sqrt{13}} \\
 \text{} & \frac{9}{2} & 5 & 1 & \frac{1}{2} & 1 & 1 & 2 \sqrt{\frac{5}{21}} \text{wr}_{4,0} \\
 \text{} & \frac{9}{2} & 5 & 1 & \frac{7}{2} & 3 & 1 & \frac{4}{7293} \left(153 \sqrt{5} \text{wr}_{4,0}+238 \sqrt{65} \text{wr}_{6,0}+168 \sqrt{85} \text{wr}_{8,0}\right) \\
 \text{} & \frac{9}{2} & 5 & 1 & \frac{9}{2} & 5 & 1 & \text{wr}_{0,0}+\frac{4}{7293} \left(1071 \text{wr}_{4,0}+544 \sqrt{13} \text{wr}_{6,0}+84 \sqrt{17} \text{wr}_{8,0}\right) \\
\hline
G_{2g} & \frac{5}{2} & 2 & 1 & \frac{5}{2} & 2 & 1 & \text{wr}_{0,0}-\frac{4 \text{wr}_{4,0}}{7} \\
 \text{} & \frac{7}{2} & 4 & 1 & \frac{5}{2} & 2 & 1 & \frac{40}{11} \sqrt{\frac{3}{13}} \text{wr}_{6,0}-\frac{20}{77} \sqrt{3} \text{wr}_{4,0} \\
 \text{} & \frac{7}{2} & 4 & 1 & \frac{7}{2} & 4 & 1 & \text{wr}_{0,0}-\frac{54 \text{wr}_{4,0}}{77}+\frac{20 \text{wr}_{6,0}}{11 \sqrt{13}} \\
 \text{} & \frac{11}{2} & 6 & 1 & \frac{5}{2} & 2 & 1 & -\frac{4}{221 \sqrt{77}} \left(170 \text{wr}_{4,0}+119 \sqrt{13} \text{wr}_{6,0}-56 \sqrt{17} \text{wr}_{8,0}\right) \\
 \text{} & \frac{11}{2} & 6 & 1 & \frac{7}{2} & 4 & 1 & \frac{2}{221} \sqrt{\frac{3}{77}} \left(170 \text{wr}_{4,0}+119 \sqrt{13} \text{wr}_{6,0}-56 \sqrt{17} \text{wr}_{8,0}\right) \\
 \text{} & \frac{11}{2} & 6 & 1 & \frac{11}{2} & 6 & 1 & \text{wr}_{0,0}+\frac{4 \text{wr}_{4,0}}{13}-\frac{8}{4199} \left(190 \sqrt{13} \text{wr}_{6,0}+35 \sqrt{17} \text{wr}_{8,0}+54 \sqrt{21}
   \text{wr}_{10,0}\right) \\
\hline
G_{2u} & \frac{5}{2} & 3 & 1 & \frac{5}{2} & 3 & 1 & \text{wr}_{0,0}-\frac{4 \text{wr}_{4,0}}{7} \\
 \text{} & \frac{7}{2} & 3 & 1 & \frac{5}{2} & 3 & 1 & \frac{20}{1001} \sqrt{3} \left(13 \text{wr}_{4,0}-14 \sqrt{13} \text{wr}_{6,0}\right) \\
 \text{} & \frac{7}{2} & 3 & 1 & \frac{7}{2} & 3 & 1 & \text{wr}_{0,0}-\frac{54 \text{wr}_{4,0}}{77}+\frac{20 \text{wr}_{6,0}}{11 \sqrt{13}} \\
 \text{} & \frac{11}{2} & 5 & 1 & \frac{5}{2} & 3 & 1 & \frac{4}{221 \sqrt{77}} \left(170 \text{wr}_{4,0}+119 \sqrt{13} \text{wr}_{6,0}-56 \sqrt{17} \text{wr}_{8,0}\right) \\
 \text{} & \frac{11}{2} & 5 & 1 & \frac{7}{2} & 3 & 1 & \frac{2}{221} \sqrt{\frac{3}{77}} \left(170 \text{wr}_{4,0}+119 \sqrt{13} \text{wr}_{6,0}-56 \sqrt{17} \text{wr}_{8,0}\right) \\
 \text{} & \frac{11}{2} & 5 & 1 & \frac{11}{2} & 5 & 1 & \text{wr}_{0,0}+\frac{4 \text{wr}_{4,0}}{13}-\frac{8}{4199} \left(190 \sqrt{13} \text{wr}_{6,0}+35 \sqrt{17} \text{wr}_{8,0}+54 \sqrt{21}
   \text{wr}_{10,0}\right) \\
\hline
 H_g & \frac{3}{2} & 2 & 1 & \frac{3}{2} & 2 & 1 & \text{wr}_{0,0} \\
 \text{} & \frac{5}{2} & 2 & 1 & \frac{3}{2} & 2 & 1 & \frac{2}{7} \sqrt{6} \text{wr}_{4,0} \\
 \text{} & \frac{5}{2} & 2 & 1 & \frac{5}{2} & 2 & 1 & \text{wr}_{0,0}+\frac{2 \text{wr}_{4,0}}{7} \\
 \text{} & \frac{7}{2} & 4 & 1 & \frac{3}{2} & 2 & 1 & \frac{2}{7} \sqrt{\frac{10}{3}} \text{wr}_{4,0} \\
 \text{} & \frac{7}{2} & 4 & 1 & \frac{5}{2} & 2 & 1 & \frac{4}{1001} \left(39 \sqrt{5} \text{wr}_{4,0}+35 \sqrt{65} \text{wr}_{6,0}\right) \\
 \text{} & \frac{7}{2} & 4 & 1 & \frac{7}{2} & 4 & 1 & \text{wr}_{0,0}+\frac{6 \text{wr}_{4,0}}{77}-\frac{80 \text{wr}_{6,0}}{33 \sqrt{13}} \\
\hline
 H_u & \frac{3}{2} & 1 & 1 & \frac{3}{2} & 1 & 1 & \text{wr}_{0,0} \\
 \text{} & \frac{5}{2} & 3 & 1 & \frac{3}{2} & 1 & 1 & -\frac{2}{7} \sqrt{6} \text{wr}_{4,0} \\
 \text{} & \frac{5}{2} & 3 & 1 & \frac{5}{2} & 3 & 1 & \text{wr}_{0,0}+\frac{2 \text{wr}_{4,0}}{7} \\
 \text{} & \frac{7}{2} & 3 & 1 & \frac{3}{2} & 1 & 1 & \frac{2}{7} \sqrt{\frac{10}{3}} \text{wr}_{4,0} \\
 \text{} & \frac{7}{2} & 3 & 1 & \frac{5}{2} & 3 & 1 & -\frac{4 \left(39 \sqrt{5} \text{wr}_{4,0}+35 \sqrt{65} \text{wr}_{6,0}\right)}{1001} \\
 \text{} & \frac{7}{2} & 3 & 1 & \frac{7}{2} & 3 & 1 & \text{wr}_{0,0}+\frac{6 \text{wr}_{4,0}}{77}-\frac{80 \text{wr}_{6,0}}{33 \sqrt{13}} \\
\hline
\end{longtable*}

==> Tables/PhaseShiftValues.tex <==
\renewcommand{\arraystretch}{1.3}
\begin{longtable*}{C|CCC|CCC}
\caption{Explicit phase shift values for the lowest partial waves and their ratio in the $G_{1g}$ irrep of the rest frame and the $G_2$ irrep of the $d = (0,0,1)$ moving frame both in the cubic box.
}
\label{tab:phaseshiftvalues}
\endfirsthead
\hline \endhead
\hline \\ \endfoot
\hline \\ \endlastfoot
\toprule
&  \multicolumn{3}{C}{G_{1g}} & \multicolumn{3}{C}{G_2}\\
\hline
 k (\GeV) & \delta_{\frac{1}{2},0} \text{(deg)} & \delta_{\frac{7}{2},4} \text{(deg)} & \delta_{\frac{1}{2},0}/\delta_{\frac{7}{2},4} & \delta_{\frac{3}{2},1} \text{(deg)}& \delta_{\frac{3}{2},2}\text{(deg)} & \delta_{\frac{3}{2},1}/\delta_{\frac{3}{2},2}\\[2pt]
 \hline
 0.01 & -15.2357 & -2.9145\times 10^{-9} & 5.2276\times 10^9 & -0.909231 & -0.00141351 & 258.256 \\
 0.02 & -30.4438 & -1.4427\times 10^{-6} & 2.1102\times 10^7 & -2.55066 & -0.0428727 & 60.5545 \\
 0.03 & -45.5969 & -0.0000524477 & 869379. & -4.08039 & -0.296717 & 25.082 \\
 0.04 & -60.6686 & -0.000644988 & 94061.7 & -5.41102 & -1.09556 & 13.4015 \\
 0.05 & -75.6333 & -0.00436655 & 17321.1 & -6.54698 & -2.82493 & 8.41003 \\
 0.06 & -90.4667 & -0.0199097 & 4543.86 & -7.49801 & -5.76661 & 5.91948 \\
 0.07 & -105.146 & -0.0689223 & 1525.58 & -8.26952 & -10.0144 & 4.53363 \\
 0.08 & -119.652 & -0.19376 & 617.528 & -8.86194 & -15.4943 & 3.69535 \\
\end{longtable*}
